Replication and Exploration of Generative Retrieval over Dynamic Corpora

Generative retrieval (GR) has emerged as a promising paradigm in information retrieval (IR). However, most existing GR models are developed and evaluated using a static document collection, and their performance in dynamic corpora where document collections evolve continuously is rarely studied. In this paper, we first reproduce and systematically evaluate various representative GR approaches over dynamic corpora. Through extensive experiments, we reveal that existing GR models with \textit{text-based} docids show superior generalization to unseen documents. We observe that the more fine-grained the docid design in the GR model, the better its performance over dynamic corpora, surpassing BM25 and even being comparable to dense retrieval methods. While GR models with \textit{numeric-based} docids show high efficiency, their performance drops significantly over dynamic corpora. Furthermore, our experiments find that the underperformance of numeric-based docids is partly due to their excessive tendency toward the initial document set, which likely results from overfitting on the training set. We then conduct an in-depth analysis of the best-performing GR methods. We identify three critical advantages of text-based docids in dynamic corpora: (i) Semantic alignment with language models' pretrained knowledge, (ii) Fine-grained docid design, and (iii) High lexical diversity. Building on these insights, we finally propose a novel multi-docid design that leverages both the efficiency of numeric-based docids and the effectiveness of text-based docids, achieving improved performance in dynamic corpus without requiring additional retraining. Our work offers empirical evidence for advancing GR methods over dynamic corpora and paves the way for developing more generalized yet efficient GR models in real-world search engines.

==> Sections/02-relatedwork.tex <==
\section{Related Work}
\subsection{Generative retrieval} 
Generative retrieval is an emerging paradigm in information retrieval that reformulates the retrieval process as a text generation task. Instead of relying on dense or sparse index structures, GR methods leverage autoregressive language models (e.g., T5) to produce a document identifies (docid)~\cite{de2020autoregressive, tay2022transformer, zhou2022dynamicretriever}.
Early work in this direction includes autoregressive entity retrieval models that generate entity titles~\cite{de2020autoregressive}.
Beyond simple string identifiers, recent studies have explored generating more semantically meaningful docids.
Existing GR methods can be categorized into two main types according to the nature of the docids: \textit{numeric-based} and \textit{text-based}.

\textit{numeric-based} docids typically involve a quantizer that converts document content into a numeric sequence, followed by training a model to learn the mapping between the document and the numeric sequence.
There are various types of quantization strategies, such as hierarchical k-means, product quantization (PQ), residual quantization (RQ), etc.
\citet{tay2022transformer} use hierarchical k-means clustering on document embeddings to generate docids and then trains the model to generate the corresponding numeric sequences.
\citet{wang2022neural} adopt a similar docids design to DSI~\cite{tay2022transformer} but applies distinct word embeddings for the same numeric value based on different positions and prefixes.
\citet{zhou2022ultron} employ PQ to convert document embeddings into numeric sequences and designs a three-stage training task to enable the model to memorize the documents.
\citet{zeng2024scalable} use RQ to quantize document embeddings, while incorporating interaction information between the query and the document when obtaining the document embeddings.
\citet{sun2024learning} adopt a variant of the RQ strategy, replacing the word embedding matrix with a codebook from the RQ method. The authors use constrained cluster centers as docids and trains the docids representations through document tokenization, retrieval, and reconstruction tasks.

\textit{Text-based} docids use meta-information from the document, such as URLs, titles, or queries, as docids, effectively utilizing the powerful capabilities of pre-trained language models. 
\citet{de2020autoregressive, chen2022gere, chen2022corpusbrain} treat the document title as the docids, as the title is the most intuitive and commonly used form of abstract textual information.
\citet{zhou2022ultron, tang2024generative} use URLs and queries as docids in web search scenarios.
Single docids type may not fully represent the information contained in a document. \citet{li2023multiview} treat various textual elements as docids and retrieves results for multiple docids simultaneously during the retrieval stage.
N-grams are also an effective way to represent document content, but directly storing n-grams for constrained decoding requires significant computational and storage costs. \citet{bevilacqua2022autoregressive} introduce the use of FM-index to store n-gram information and control generation, significantly improving both efficiency and retrieval performance.

In this paper, we reproduce representative methods from both \textit{numeric-based} and \textit{text-based} paradigms to comprehensively evaluate their adaptability in dynamic corpora.


\subsection{GR over dynamic corpora}
Previous GR methods primarily focus on fixed document collections, whereas practical tasks often involve corpora that continuously evolve over time.
To address this challenge, researchers have developed a series of methods to optimize GR models for handling dynamic corpora.
\citet{mehta2022dsi++} employ an incremental training method by optimizing flat loss basins through the Sharpness-Aware Minimization (SAM) optimizer, enabling the model to remember new documents while maintaining stable retrieval performance for the initial documents.
\citet{guo2024corpusbrain++} design an adapter structure that shares a backbone model while introducing task-specific adapters for training on specific documents. This method effectively learns representations for new documents.
\citet{chen2023continual} build upon the PQ strategy and proposes Incremental Product Quantization (IPQ), using the generated PQ codes as docids. It achieves flexible document addition by updating the PQ centroids.
\citet{kim2023exploring} evaluate the performance of GR methods on dynamic corpora, demonstrating the superiority of GR in terms of efficiency and memory compared to traditional retrieval strategies.

These methods have, to some extent, addressed or alleviated the challenges faced by GR methods in dynamic corpora tasks. However, they either require additional training or involve complex docids designs, making them unsuitable for the demands of dynamic corpora in practical scenarios. Therefore, it is crucial to explore the ability of models to generalize to new documents without complex modifications or additional training.

